Global Rhythm Style Transfer Without Text Transcriptions

Prosody plays an important role in characterizing the style of a speaker or an emotion, but most non-parallel voice or emotion style transfer algorithms do not convert any prosody information. Two major components of prosody are pitch and rhythm. Disentangling the prosody information, particularly the rhythm component, from the speech is challenging because it involves breaking the synchrony between the input speech and the disentangled speech representation. As a result, most existing prosody style transfer algorithms would need to rely on some form of text transcriptions to identify the content information, which confines their application to high-resource languages only. Recently, SpeechSplit has made sizeable progress towards unsupervised prosody style transfer, but it is unable to extract high-level global prosody style in an unsupervised manner. In this paper, we propose AutoPST, which can disentangle global prosody style from speech without relying on any text transcriptions. AutoPST is an Autoencoder-based Prosody Style Transfer framework with a thorough rhythm removal module guided by the self-expressive representation learning. Experiments on different style transfer tasks show that AutoPST can effectively convert prosody that correctly reflects the styles of the target domains.

==> background_old.tex <==
% ------------------- Version with less math -----------------------
In this section, we will provide some background information on why disentangling rhythm has been difficult.
% , and on why the previous attempts can fail in some scenarios.

\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{figs/spect.pdf}
\caption{Mel-spectrograms of two utterances of \emph{``Please call Stella''} with different speech rates. The phone segments are marked on the $x$-axis. The grey dashed lines between the two spectrograms mark the phone alignment, which shows that the changes in duration are disproportional across different phones.}
\label{fig:sepct}
\end{figure}

\subsection{Rhythm Information}

% Rhythm is reflected by the duration of each pronunciation unit in speech. 
Figure~\ref{fig:sepct} shows two utterances of the same word \emph{``Please call Stella''}, with the phone segments marked on the $x$-axis. As shown, although the content is almost the same across the two utterances, each phone in the second utterance is repeated for more frames than in the first utterance. In this paper, we will measure rhythm as the number of frame-aligned repetitions of each phone symbol. 

Therefore, the task of disentangling rhythm involves removing phone repetitions while retaining phone identities.
% , uncovering the ground truth phone sequence \emph{without repetitions}. 
If the text transcriptions were available, this could be achieved by training an asynchronous sequence-to-sequence model, such as the Transformer \cite{vaswani2017attention}, to predict the phone sequence from input speech. However, without the phonetic labels, it remains an unresolved challenge to uncover the phonetic units in an unsupervised manner.

\subsection{Disentangling Rhythm by Resampling}
\label{subsec:segment}

Existing unsupervised rhythm disentanglement techniques seek to obscure the rhythm information by temporally resampling the speech sequence or its hidden representation sequence. One common resampling strategy, as proposed by \citet{polyak2019attention}, involves three steps. First, the input sequence is separated into segments of random lengths. Second, for each segment, a sampling rate is randomly drawn from some distribution. Finally, the corresponding segment is resampled at this sampling rate.
% (equivalent to uniformly stretching each segment to a random length). 

% Durations sampled at random do not need to be 
% sampled {\em uniformly} at random.
To gauge how much rhythm information the random resampling can remove, consider two hypothetical speech sequences, where everything is the same except for the rhythm. Namely, they have the same content but are temporally unaligned. If random resampling is to reduce the 
rhythm information in each utterance,
%If the rhythm information is to be reduced at all, 
there must be a non-zero probability that the random resampling temporally aligns them (hence making them identical because their only difference is rhythm). Thus, the original rhythm information distinguishing the two utterances is removed. Formally, denote \e{\tilde{\bm Z}(t)} and \e{\tilde{\bm Z}'(t)} as the resampled outputs of the two unaligned but otherwise identical sequences. Then a necessary condition for reduction in rhythm information is that
\begin{equation}
\small
    Pr(\tilde{\bm Z}(t) = \tilde{\bm Z}'(t)) > 0.
    \label{eq:nes_cond}
\end{equation}
% Random resampling, with non-uniform randomness, 
% can be trained to maximize the probability in
% Eq.~(\ref{eq:nes_cond}).
Higher probability removes more rhythm information. If the probability becomes one, all the rhythm information distinguishing the two utterances is completely lost.

Therefore, we argue that the above random resampling algorithm does not remove much rhythm information, because it has a low probability of aligning any utterance pairs with the same content but different rhythm patterns. Figure~\ref{fig:sepct} is a counterexample, where the duration of each phone changes disproportionally. The vowel ``ea'' gets more stretched than the consonants. Consider the case where the entire sequence falls into one random segment in the first step of the resampling algorithm. Then, due to the disproportional stretch among the phones, it is impossible to simultaneously align all the phones by uniformly stretching or squeezing the two utterances. If the utterances are broken into multiple random segments, it is possible to achieve the alignment, but this requires the number of random segments is greater than or equal to the number of phones, with at least one segment boundary between each pair of phone boundaries, whose probability of occurring is extremely low.
In short, 
% to overcome the limitation of the existing resampling scheme, 
we need better ways to account for the disproportional variations in duration across different phones.


% ------------------- Version with more math -----------------------
% To assist a better understanding of the design motivations behind \algname, in this section, we will provide some background information on why disentangling rhythm has been difficult, and on why the previous attempts can fail in some scenarios.

% \subsection{A Simple Model of Rhythm}

% Rhythm is reflected by the duration of each pronunciation unit in speech. To formalize our analysis, we build a simplified model for the rhythm information. Denote
% \[
% \small
%     \mathcal{C} = \{c_i(t): i \in [N]\}
% \]
% as the pool of all the pronunciation units within a language, such as phones or sub-phones, uttered in a standard speech rate. For the remainder of this paper, we will assume the pronunciation units are phones. \e{c_i(t)} denotes the prototype speech signal of the $i$-th phone. \e{[N]} denotes the positive integer set up to \e{N} and \e{N} denotes the total number of phones. Then a speech utterance, denoted as \e{S(t)}, can be produced by selecting a sequence of phones and concatenating the temporally-warped prototypes together, \emph{i.e.}
% \begin{equation}
% \small
% \begin{aligned}
%     & S(t) = \mbox{concat}\Big(c_{i_1}(R_1 t), c_{i_2}(R_2 t), \cdots, c_{i_K}(R_K t)\Big).
% \end{aligned}
%     \label{eq:speech}
% \end{equation}
% concat\e{(\cdot)} denotes concatenating the sequences into a long sequence. \e{K} denotes the total number of phones within an utterance. \e{i_{1:K} \in [N]^K} is a sequence of phone identities, representing the \emph{content information}. \e{R_{1:K}} are random variables governing how fast each phone is uttered, representing the \emph{rhythm information}. The larger each value is, the faster the corresponding phone is. It is important to note that \e{R_{1:K}} are \emph{not} identically distributed, because different phones have different duration flexibility. For example, consonants generally have far less duration flexibility than vowels.

% Equation~\eqref{eq:speech} is an overly-simplified model of speech. It does not account for the other variations in speech, such as voice and pitch. Nevertheless, it is sufficient for the purpose of analyzing rhythm disentanglement. According to this model, the task of disentangling rhythm involves removing the information of \e{R_{1:K}} while retaining the phone identities \e{i_{1:K}}. Therefore, the most ideal way of removing rhythm is to directly uncover the ground truth phone sequence \emph{without repetitions}. If the text transcriptions were available, this could be easily achieved by training an asynchronous sequence-to-sequence model, such as the Transformer \cite{xx}, to predict the phoneme sequence from input speech. However, without the phonetic labels, it remains an unresolved challenge to uncover the phonetic units in an unsupervised manner.

% \subsection{Existing Unsupervised Rhythm Disentanglement Techniques}
% \label{subsec:segment}

% Alternatively, the existing unsupervised rhythm disentanglement techniques seek to obscure the rhythm information by temporally resampling the input or representation sequence. One common resampling strategy is to randomly break the input sequence into segments of random lengths, and then resample each segment with a random resampling rate \cite{xx}. Formally, the output of the resampling module, \e{\hat{S}(t)}, can be expressed as
% \begin{equation}
% \small
%     \tilde{S}(t) = S(L t), \quad \mbox{for some random variable } L.
% \end{equation}
% Here we are assuming \e{\hat{S}(t)} and \e{S(\lambda t)} are both continuous-time variables for ease of illustration and analysis. In practice, we can use interpolation to accommodate non-integer $t$.

% One necessary condition for the rhythm information to be reduced at all is that for any speech pairs with the same content but different rhythm patterns, there exists a non-zero probability that they are mapped to the same sequence after resampling. If this happens, it would be impossible to fully recover the rhythm only based on the resampling output. Formally, for two particular instances of speech
% \begin{equation}
%     \begin{aligned}
%         & s(t) = [c_{i_1}(r_1 t), c_{i_2}(r_2 t), \cdots c_{i_K}(r_K t)] \\
%         & s'(t) = [c_{i_1}(r'_1 t), c_{i_2}(r'_2 t), \cdots c_{i_K}(r'_K t)],
%     \end{aligned}
% \end{equation}
% where \e{r_{1:K}} and \e{r'_{1:K}} denote two different realizations of \e{R_{1:K}}. Then the necessary condition states that
% \begin{equation}
%     \exists l, l', \quad \mbox{s.t.} \quad s(lt) = s'(l't).
%     \label{eq:nes_cond}
% \end{equation}
% Unfortunately, the aforementioned random resampling strategy does not satisfy Equation~\eqref{eq:nes_cond}. Figure~\ref{xx} shows a simple counter-example, where there are two speech utterances of the same two-phone sequence. The first phone is a consonant and the second is a vowel. The second utterance is longer than the first. As discussed, only the vowel gets stretched and the consonant stays the same. Due to the disproportional stretch between the two phones, it is impossible to match the duration of both phones by uniformly stretching or squeezing the two utterances. As a result, the two rhythm patterns will always be distinguishable.

% As can be concluded from the discussion above, in order to overcome the limitation of the existing resampling scheme, we must find ways to account for the disproportional variations in duration across different phones.
